Speaker Verification in Agent-Generated Conversations

The recent success of large language models (LLMs) has attracted widespread interest to develop role-playing conversational agents personalized to the characteristics and styles of different speakers to enhance their abilities to perform both general and special purpose dialogue tasks. However, the ability to personalize the generated utterances to speakers, whether conducted by human or LLM, has not been well studied. To bridge this gap, our study introduces a novel evaluation challenge: speaker verification in agent-generated conversations, which aimed to verify whether two sets of utterances originate from the same speaker. To this end, we assemble a large dataset collection encompassing thousands of speakers and their utterances. We also develop and evaluate speaker verification models under experiment setups. We further utilize the speaker verification models to evaluate the personalization abilities of LLM-based role-playing models. Comprehensive experiments suggest that the current role-playing models fail in accurately mimicking speakers, primarily due to their inherent linguistic characteristics.

==> latex/evaluation_by_other_models.tex <==
\section{The Evaluations by Other Models}
\label{sec:appendix2}

We utilized various speaker verification methods to assess the performance of role-playing models. As the reliability of out-of-box models are uncertain, we show similarity score distributions between real utterance pairs on evaluation datasets. As shown in Figures~\ref{fig:real-real-out-of-box}, the out-of-box models struggle to distinguish between speakers. This observation aligns with our previous findings. Tables~\ref{tab:out-of-box score} and~\ref{tab:fine tuned score} present the simulation and distinction scores from different evaluators, while Figures~\ref{fig:liwc-pairs} to~\ref{fig:luar-ft-pairs} illustrate the distribution of these similarity scores. Both the scores and their distributions suggest that current LLM-based role-playing models fall short in accurately simulating roles, particularly in aspects like linguistic style. Conversely, these models tend to maintain their own distinctive style during role-play.


\begin{figure*}[tb]
  \centering
  \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figs/real-real-lsm.png}
    \caption{LIWC}
  \end{subfigure}
  \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figs/real-real-lisa.png}
    \caption{LISA}
  \end{subfigure} 
  \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figs/real-real-STEL.png}
    \caption{STEL}
  \end{subfigure}
  \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figs/real-real-SBERT.png}
    \caption{SBERT}
  \end{subfigure}
  \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figs/real-real-LUAR.png}
    \caption{LUAR}
  \end{subfigure}
  \caption{The similarity scores, derived from the out-of-box models of real utterance pairs across two test sets.}
  \label{fig:real-real-out-of-box}
\end{figure*}

% \begin{figure*}[tb]
%   \centering
%   \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figs/real-real-STEL_finetune.png}
%     \caption{Fine Tuned STEL}
%   \end{subfigure}
%   \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figs/real-real-SBERT_finetune.png}
%     \caption{Fine Tuned SBERT}
%   \end{subfigure} 
%   \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figs/real-real-roberta_finetune.png}
%     \caption{Fine Tuned RoBERTa}
%   \end{subfigure}
%   \begin{subfigure}{0.24\textwidth}
%     \includegraphics[width=\textwidth]{figs/real-real-LUAR_finetune.png}
%     \caption{Fine Tuned LUAR}
%   \end{subfigure}
%   \caption{The similarity scores, derived from the fine tuned models of real utterance pairs across two test sets.}
%   \label{fig:real-real-fine tuned}
% \end{figure*}

\begin{table*}[tb]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{LIWC} & \multicolumn{2}{c}{LISA} & \multicolumn{2}{c}{STEL} & \multicolumn{2}{c}{SBERT} & \multicolumn{2}{c}{LUAR} \\
\multicolumn{1}{c}{}                        & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$  & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$  \\ \midrule
LLaMA2-Chat-7B      & 62.80      & 41.45       & 91.20      & 5.98       & 9.93       & 29.17       & 42.49       & 69.95       & 88.84      & 8.12      \\
LLaMA2-Chat-13B     & 52.35      & 54.61       & 90.64      & 5.17       & 12.77      & 33.45       & 42.88       & 67.79       & 87.91      & 8.60       \\
LLaMA2-Chat-70B     & 65.52      & 25.38       & 88.75      & 8.46       & 40.49      & 20.11       & 39.55       & 71.04       & 88.95      & 9.98   \\
ChatHaruhi          & 62.61      & 34.95       & 87.04      & 7.72       & 43.15      & 16.43       & 44.63       & 62.25       & 86.40      & 13.16     \\
RoleGPT             & 58.57      & 41.18       & 86.06      & 9.76       & 52.71      & 21.2       & 42.23       & 65.26       & 81.53      & 20.19   \\ \hline
CharacterLLM        & 56.97      & 37.41       & 79.91      & 15.47       & 18.17     & 48.99       & 27.29       & 70.11       & 68.53      & 28.64    \\
Character.AI        & 61.06      & 48.96       & 81.46      & 19.2       & 47.42      & 49.62       & 49.72       & 59.12       & 88.94      & 27.31     \\ \bottomrule
\end{tabular}}
\caption{The simulation and distinction score by out-of-box models.}
\label{tab:out-of-box score}
\end{table*}

\begin{table*}[tb]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{STEL$_{ft}$} & \multicolumn{2}{c}{SBERT$_{ft}$} & \multicolumn{2}{c}{RoBERTa$_{ft}$} & \multicolumn{2}{c}{LUAR$_{ft}$} \\
\multicolumn{1}{c}{}     & Simulation$\uparrow$   & Distinction$\uparrow$  & Simulation$\uparrow$   & Distinction$\uparrow$   & Simulation$\uparrow$    & Distinction$\uparrow$    & Simulation$\uparrow$   & Distinction$\uparrow$  \\ \midrule
LLaMA2-Chat-7B           & 42.55        & 58.15        & 47.04        & 73.35         & 51.85         & 64.32          & 50.20        & 58.46        \\
LLaMA2-Chat-13B          & 42.71        & 50.48        & 45.49        & 64.18         & 48.65         & 56.77          & 40.56        & 42.79        \\
LLaMA2-Chat-70B          & 47.21        & 61.60        & 54.26        & 70.24         & 57.18         & 66.97          & 56.98        & 50.89        \\
ChatHaruhi               & 44.13        & 49.22        & 51.28        & 64.64         & 37.81         & 47.61          & 57.69        & 37.66        \\
RoleGPT                  & 55.80        & 53.72        & 66.45        & 62.30         & 59.83         & 62.19          & 61.79        & 46.42        \\ \hline
CharacterLLM             & 42.91        & 26.90        & 51.12        & 61.49         & 46.90         & 54.41          & 55.49        & 33.13        \\
Character.AI             & 58.22        & 49.76        & 57.27        & 48.15         & 55.68         & 50.66          & 60.34        & 51.00        \\ \bottomrule
\end{tabular}}
\caption{The simulation and distinction score by fine-tuned models.}
\label{tab:fine tuned score}
\end{table*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lsm-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lsm-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on LIWC.}
  \label{fig:liwc-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lisa-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lisa-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on LIAS.}
  \label{fig:lisa-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on STEL.}
  \label{fig:stel-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on SBERT.}
  \label{fig:sbert-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on LUAR.}
  \label{fig:luar-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL_finetune-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL_finetune-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on STEL$_{ft}$.}
  \label{fig:stel-ft-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT_finetune-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT_finetune-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on SBERT$_{ft}$.}
  \label{fig:sbert-ft-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/roberta_finetune-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/roberta_finetune-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on RoBERTa$_{ft}$.}
  \label{fig:roberta-ft-pairs}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR_finetune-real-generated.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR_finetune-generated-generated.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of role-playing models based on LUAR$_{ft}$.}
  \label{fig:luar-ft-pairs}
\end{figure*}

==> latex/evaluation_on_persona_chatbot.tex <==
\section{Evaluations on Persona Chatbot}

In addition to evaluating role-playing models based on Large Language Models (LLMs), our assessment extends to persona chatbots through our proposed models. Specifically, we incorporate a prompt-based model, PersonaChatGen~\citep{leePERSONACHATGENGeneratingPersonalized2022}, and two persona chatbot models, PersonaGPT~\citep{tang2021persona} and TransferTransfo~\citep{wolf2019transfertransfo}, into our evaluation framework. Additionally, we include MBTI-S2Conv~\citep{tuCharacterChatLearningConversational2023}, a dataset facilitating personalized social support conversations generated by CharacterChat, featuring dialogues among characters exhibiting distinct MBTI persona traits. To provide persona information for persona chatbots, we sample 500 personas from the PersonaChat dataset~\citep{zhang2018personalizing}. As indicated in Table~\ref{tab:dist-persona-out-of-box} and Table~\ref{tab:dist-persona-ft}, both simulation and distinction scores significantly surpass those observed in role-playing scenarios. However, it's noteworthy that distinction scores for the PersonaChat dataset are also exceptionally high. Upon manual review of the dataset, we observe that the linguistic style of persona chat tends to be bland, exemplified by expressions such as "me too.", "I love dogs", and "I am writing an ebook about them". This simplicity in language may contribute to the ease of simulation and the elevated distinction scores observed. Aligned with prior observations, the distinction scores for the prompt-based LLM model, specifically CharacterChat, surpass those of other models. This trend suggests that the LLM inherently possesses its distinct character, potentially hindering its ability to effectively mimic varied personalized traits. Figure~\ref{fig:liwc-pairs-persona} to Figure~\ref{fig:luar-ft-pairs-persona} show the distribution of similarity scores across persona chatbots.

\begin{table*}[tb]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{LIWC} & \multicolumn{2}{c}{LISA} & \multicolumn{2}{c}{STEL} & \multicolumn{2}{c}{SBERT} & \multicolumn{2}{c}{LUAR} \\
\multicolumn{1}{c}{}                        & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$ & Simulation$\uparrow$  & Distinction$\uparrow$ & Simulation$\uparrow$ & Distinction$\uparrow$  \\ \midrule
PersonaChat         & -          & 32.06       & -          & 13.5       & -          & 4.44       & -           & 56.34       & -          & 26.96      \\ \hline
PersonaGPT          & 68.76      & 29.40       & 87.45      & 9.76       & 82.12      & 4.17       & 48.46       & 43.8       & 69.53      & 26.13      \\
TransferTransfo     & 67.34      & 31.48       & 87.85      & 7.70       & 77.91      & 5.09       & 48.45       & 40.39       & 80.80      & 21.07      \\
PersonaChatGen      & 53.06      & 28.27       & 81.86      & 6.67       & 43.62      & 9.86       & 35.64       & 43.97       & 60.87      & 24.96      \\ \hline
CharacterChat       & -          & 23.35       & -          & 4.70       & -          & 10.5       & -           & 36.64       & -          & 12.03      \\ \bottomrule
\end{tabular}}
\caption{The simulation and distinction score by out-of-box models. As the PersonaChat and CharacterChat dataset do not consist of enough conversations from the same speakers, we only evaluate the distinction scores.}
\label{tab:dist-persona-out-of-box}
\end{table*}

\begin{table*}[tb]
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{2}{c}{STEL$_{ft}$} & \multicolumn{2}{c}{SBERT$_{ft}$} & \multicolumn{2}{c}{RoBERTa$_{ft}$} & \multicolumn{2}{c}{LUAR$_{ft}$}  & \multicolumn{2}{c}{Mixed Features} \\
\multicolumn{1}{c}{}     & Simulation$\uparrow$   & Distinction$\uparrow$  & Simulation$\uparrow$   & Distinction$\uparrow$   & Simulation$\uparrow$    & Distinction$\uparrow$    & Simulation$\uparrow$   & Distinction$\uparrow$     & Simulation$\uparrow$   & Distinction$\uparrow$  \\ \midrule
PersonaChat           & -            & 7.58        & -            & 30.48         & -             & 25.61          & -            & 26.28          & -            & 22.74        \\ \hline
PersonaGPT            & 80.24        & 9.79        & 71.63        & 24.78         & 74.85         & 22.74          & 69.33        & 25.12          & 74.01        & 20.61        \\
TransferTransfo       & 76.89        & 10.38        & 68.70        & 28.34         & 72.48         & 25.93          & 67.70        & 26.00          & 71.44        & 22.66        \\
PersonaChatGen        & 53.42        & 19.85        & 69.22        & 27.25         & 71.31         & 26.71          & 62.30        & 24.88          & 64.03        & 24.67        \\ \hline
CharacterChat         & -            & 6.29        & -            & 24.91         & -             & 20.10          & -            & 15.02          & -            & 16.58        \\ \bottomrule
\end{tabular}}
\caption{The simulation and distinction score by fine-tuned models.  As the PersonaChat and CharacterChat dataset do not consist of enough conversations from the same speakers, we only evaluate the distinction scores.}
\label{tab:dist-persona-ft}
\end{table*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lsm-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lsm-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on LIWC.}
  \label{fig:liwc-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lisa-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/lisa-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on LIAS.}
  \label{fig:lisa-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on STEL.}
  \label{fig:stel-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on SBERT.}
  \label{fig:sbert-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on LUAR.}
  \label{fig:luar-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL_finetune-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/STEL_finetune-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on STEL$_{ft}$.}
  \label{fig:stel-ft-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT_finetune-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/SBERT_finetune-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on SBERT$_{ft}$.}
  \label{fig:sbert-ft-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/roberta_finetune-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/roberta_finetune-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on RoBERTa$_{ft}$.}
  \label{fig:roberta-ft-pairs-persona}
\end{figure*}

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR_finetune-real-generated-persona.png}
    \caption{Real-Generated Pairs}
  \end{subfigure}\\
  \begin{subfigure}{\textwidth}
    \includegraphics[width=\textwidth]{figs/LUAR_finetune-generated-generated-persona.png}
    \caption{Generated-Generated Pairs}
  \end{subfigure} 
  \caption{The similarity score distribution of real-generated and generated-generated pairs of persona chatbots based on LUAR$_{ft}$.}
  \label{fig:luar-ft-pairs-persona}
\end{figure*}

==> latex/impact_of_utter_number.tex <==
\section{The Impact from Utterances Number for Speaker Verification}
\label{sec:appendix1}
As more utterance may provide more personal information, we evaluate the impact from the number of utterances in pairs. We focus on the results within the Unseen-Unseen set at the Hard level to investigate the relationship between verification performance (measured by AUC score) and conversation length (number of turns). Figure~\ref{fig:utter} presents the AUC score performance of each model, differentiated by model type and the number of utterances. All models demonstrate a general improvement as the number of utterances increases, though this trend is not consistently observed. Notably, there are declines at two specific points. The initial decrease observed from 5 to 20 utterances could be linked to the addition of more content that, while increasing in quantity, does not sufficiently enhance informativeness, thus complicating the verification process. This is particularly evident in models like LISA, SBERT, RoBERTa${ft}$, and SBERT${ft}$, which primarily depend on content for attribution determination. The subsequent drop at the point of longest conversations implies that an overload of utterances might introduce noise, obstructing the identification of key features crucial for precise verification. This trend is noticeable across most models, suggesting that the detrimental effect of noise from overly lengthy conversations could compromise the performance of the majority of models.

\begin{figure*}[tb]
  \centering
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{figs/style_utter_len.png}
    \caption{Style-Based Models}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{figs/authorship_utter_len.png}
    \caption{Authorship Attribution Models}
  \end{subfigure} \\
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{figs/finetune_utter_len.png}
    \caption{Fine Tuned Models}
  \end{subfigure}
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{figs/mix_utter_len.png}
    \caption{Mixed Features}
  \end{subfigure}
  \caption{AUC test performance (y-axis) across different model categories: (a) style-based models, (b) authorship attribution models, (c) fine-tuned models, and (d) mixed features models, in the Unseen-Unseen setting at the 'Hard' level of difficulty, as a function of the number of utterances per speaker (x-axis).}
  \label{fig:utter}
\end{figure*}

==> latex/speaker_verification_in_speech.tex <==
\section{Speaker Verification in Speech Processing}

Speaker verification in speech processing seeks to confirm if a voice claim matches the true identity of the speaker by comparing the voice sample against a pre-stored voiceprint. In this topic, researchers have developed methods based on neural network structures and methodologies, often leveraging both publicly available and proprietary datasets~\citep{wan2018generalized,li2021fdn,liu2023cross,kim2023analysis}. 
For example, FDN~\citep{li2021fdn} details an innovative network that layers intonation analysis atop lower-level voice embeddings, markedly boosting system precision, a claim substantiated by tests on the VoxCeleb1 dataset. Moreover, research by \citet{liu2023cross} investigates the integration of visual cues like lip movements with auditory speech, establishing a novel dual-mode learning approach in speech processing. 
Unlike the above works, our study focuses on speaker verification using conversation data and considers more evaluation settings which have not been studied, e.g., verification involving completely unseen speakers.
